Inter-Block Permuted Turbo Codes

The structure and size of the interleaver used in a turbo code critically affect the distance spectrum and the covariance property of a component decoder's information input and soft output. This paper introduces a new class of interleavers, the inter-block permutation (IBP) interleavers, that can be build on any existing "good" block-wise interleaver by simply adding an IBP stage. The IBP interleavers reduce the above-mentioned correlation and increase the effective interleaving size. The increased effective interleaving size improves the distance spectrum while the reduced covariance enhances the iterative decoder's performance. Moreover, the structure of the IBP(-interleaved) turbo codes (IBPTC) is naturally fit for high rate applications that necessitate parallel decoding. We present some useful bounds and constraints associated with the IBPTC that can be used as design guidelines. The corresponding codeword weight upper bounds for weight-2 and weight-4 input sequences are derived. Based on some of the design guidelines, we propose a simple IBP algorithm and show that the associated IBPTC yields 0.3 to 1.2 dB performance gain, or equivalently, an IBPTC renders the same performance with a much reduced interleaving delay. The EXIT and covariance behaviors provide another numerical proof of the superiority of the proposed IBPTC.

==> Introduction.tex <==
\section{Introduction}
The turbo code's extraordinary performance is in part due to a
class of suboptimal iterative decoding algorithms that generate
soft outputs based on the maximum a posteriori (MAP) principle. At
each decoding round, an a posteriori probability (APP) decoder
provides extrinsic information for use in the ensuing round as the
a priori information. The extrinsic information about an
information bit is gathered through message-passing from the
channel output samples corresponding to other related bits, and
its derivation is based on the structures of the interleaver and
the component codes as well as the statistical property of the
channel. The interleaver is thus an integrated and critical
component of a turbo code (TC) and its importance has been well
documented.

As the interleaver is of finite size, say, $L$ bits, the input
information sequence is segmented into blocks of $L$ bits, leading
to separate encoding, interleaving and decoding of each block. As
a result, the message-passing process induced by the interleaver
is confined to within a block. Given the component codes and the
decoding algorithm, performance can be improved by increasing the
interleaver (block) size.

At the cost of prolonged interleaver delay, the increased block
size not only enables the decoder to gather the extrinsic
information from more (noisy) data and parity samples but also
makes it easier to reduce the covariance between the extrinsic
(information) outputs and the corresponding information inputs,
which, as suggested by Hokfelt {\it et al.} \cite{Hokfelt} and
Sadjadpour {\it et al.} \cite{Harnid}, is a desired attribute of
the interleaver/deinterleaver pair. Intuitively the less
covariance between information input and extrinsic output the more
`new' information the extrinsic output would carry over to the new
APP decoding round, where two consecutive decoding rounds
constitute a decoding iteration. Increasing the interleaver size
also provides greater flexibility in designing a better
permutation rule to avoid generating low weight codewords and to
improve the free distance and spectrum properties of the
associated turbo code \cite{Shamai}, \cite{Wang}.

In short, the interleaver and the component codes' structures
together determine the distance spectrum of the code and, through
the message-passing process embedded in the iterative decoding
procedure, determine the bit error performance. In this paper, we
present a new interleaver structure that serves both purposes
without increasing the total interleaving delay if certain degrees
of parallelism are allowed and a proper decoding schedule is in
place.


Before formally defining our interleaver structure, we give a
tutorial explanation for its effectiveness in expanding an
iterative decoder's message-passing range. Consider the
interleaver structure shown in Fig. 1. A data sequence is
partitioned into $L$-bit blocks, each block being represented by a
rectangular. Information bits are first permuted within their
respective blocks. After such intra-block permutations, bits
within a block are further systematically permuted with those in
other neighboring blocks. It is obvious that the additional
inter-block permutation (IBP) leads to progressively larger ranges
for message-passing as the number of decoding iteration increases.
Intuitively, when the extrinsic information about a particular
information bit is gathered from more and farther data and parity
samples, it becomes more reliable and less correlated with the
information bit. Let us elaborate on this message-passing process
associated with the iterative decoding of an IBP-interleaved turbo
code (IBPTC).

In general, a turbo code may consist of several parallel
constituent codes and interleavers. For simplicity of
presentation, however, we will consider only the classic turbo
codes that use two identical recursive systematic convolutional
component codes and one interleaver in the subsequent discussion.
Fig. \ref{fig:factor_graph} is a graph representation that
illustrates the behavior of such a classic turbo code that uses an
IBP interleaver (IBPI). In this figure, nodes $U_i, U_i'$
represent a data block of length $L$ and its permuted version.
$X^0_i, X^1_i, X^2_i$ denote the uncoded (systematic part) and two
encoded blocks while $Y^0_i,Y^1_i,Y^2_i$ are the corresponding
received blocks. The bold solid lines connecting $U_i$ and $U_i'$
indicate intra-block permutations that confine permuted bits to
within the same block. An IBP that permutes bits of a given block
with some of those bits within the two immediate adjacent blocks
and the original block is represented by the dotted lines
connecting $U_i$ and $\{U_{i+1}, U_i, U_{i-1}\}$. Both solid and
dotted lines also represent directions of information flow to and
from a node during an iterative decoding process.

Take node $U_3$ as an example and, for the convenience of
describing the decoding process, refer to the decoder responsible
for decoding node $U_i$ or the corresponding codeword $(X^0_i,
X^1_i)$\footnote{For brevity, we shall make no distinction between
$U_i$ (or $U_i'$) and its associated codeword if there is no
danger of confusion.} as the first APP decoder and that in charge
of decoding $U_i'$ or its associated codeword the second APP
decoder--although physically they might be the same one. After the
first APP decoding of node $U_3$, the associated extrinsic
information is passed to nodes $U_2'$, $U_3'$ and $U_4'$ by the
interleaver. When the second APP decoder is decoding the $U_2'$
($U_4'$) block, it uses extrinsic information derived from $U_3$,
along with that derived from $U_1$ and $U_2$ ($U_4$, $U_5$), as
the a priori information to generate new extrinsic information,
after de-interleaving, to nodes $\{U_1, U_2, U_3\}$ ($\{U_3, U_4,
U_5\}$). We see that, after just one iteration the information
associated with the $U_3$ block has already been passed to
portions of four neighboring blocks and $U_3$ itself. Therefore,
when the first APP decoder is decoding node $U_3$ for the second
time it can use information collected from these four adjacent
blocks. As one proceeds with further iterations, more information
will be available for the APP decoder while, as we shall see in
the next section, the interleaving delay can be kept at a fixed
$2L$ bits, and, more importantly, the average decoding delay per
block can remain invariant if certain conditions are satisfied.

This last property is critically important, for it implies that an
IBP interleaver can have an unbounded equivalent interleaving
depth (size) that is constrained only by the number of turbo
decoding iterations and the data sequence duration while keeping
the average interleaving and decoding delay bounded by its local
interleaving depth.


The rest of this paper is organized as follows: In Section II, we
introduce the structure of IBP interleavers and define the related
parameters. In section III, latency and implementation issues are
discussed. Some important codeword weight bounds and intra-block
interleaver constraints associated with the IBPTC are derived in
Section IV. When deriving these bounds, we first assume no
knowledge of the intra-block permutation then obtain some
constraints on the intra-block permutation to avoid producing
low-weight codewords. In Section V, we consider the problem of
joint intra-block and inter-block permutation design and derive an
upper-bound for the achievable minimum distance. Some of the
properties derived in Sections IV and V can be used as the IBPI
design guidelines. Architecture for realizing IBPTC and an IBP
algorithm are presented in Section VI, so is a modified
semi-random interleaver which serves as the intra-block
interleaver. In Section VII, we provide simulation results to
validate our assertion that our proposal does yield significant
improvement. The final section summarizes our work and gives some
concluding remarks.


==> Table_Figure.tex <==

\begin{table}
  \centering
  \caption{IBP Algorithm}\label{Algorithm1}
\begin{tabular}{|l|} \hline
\underline{Variables}\\
L-block length\\
N-total number of blocks\\
K-block number index\\
D(m,k)-data on the $k$th block $m$th position\\
\underline{Recursion}\\
for K=0 to N-1\\
\hspace{0.5cm} for i=0 to i=S-1\\
\hspace{1.0cm} if (K-i $>$ 0)\\
\hspace{1.5cm} if (K mod (2$\cdot$(i+1)) $<$ i+1)\\
\hspace{2.0cm} set m=2$\cdot$i+1\\
\hspace{1.5cm} else\\
\hspace{2.0cm} set m=2$\cdot$i+2\\
\hspace{1.5cm} end\\
\hspace{1.5cm} while (m $<$ L)\\
\hspace{2.0cm} swap D(m,K) and D(m,K-i-1)\\
\hspace{2.0cm} set m=m+2S+1\\
\hspace{1.5cm} end\\
\hspace{1.0cm} end\\
\hspace{0.5cm} end\\
end\\
\hline
\end{tabular}
\end{table}

\begin{figure}[ht]
\begin{center}
\hspace{0.0mm} \vspace{0.0cm} \epsfxsize=100mm
\epsffile{example.eps}
%\includegraphics[totalheight=8.0cm]{example.eps}
\caption{ An inter-block permutation interleaving procedure. }
\label{fig:example} \vspace{0.0mm}
\end{center}
\end{figure}

\begin{figure}[ht]
\begin{center}
\hspace{0.0mm} \vspace{0.0cm} \epsfxsize=80mm
\epsffile{factor_graph_IT.eps} \caption{Factor graph
representation and information flow of an IBPTC and a classic TC.}
\label{fig:factor_graph} \vspace{0.0mm}
\end{center}
\end{figure}

\begin{figure}[ht]
\begin{center}
\hspace{0.0mm} \vspace{0.0cm} \epsfxsize=60mm
\epsffile{Scheduling_Comparison.eps} \caption{A comparison of
exemplary decoding schedules for classic TC and IBPTC when
decoding 7 blocks with 2 iterations (four decoding rounds). The
numbers in the two rectangular grid-like tables represent the
order the APP decoder performs decoding. Hence the first block of
the classic TC is decoded by the first 4 decoding rounds (the
leftmost column) but that of the IBPTC is decoded by the first,
third, sixth and tenth decoding rounds; see Section III for
detailed discussion.} \label{fig:scheduling_comparison}
\vspace{0.0mm}
\end{center}
\end{figure}

\begin{figure}[ht]
\begin{center}
\hspace{0.0mm} \vspace{0.0cm} \epsfxsize=70mm
\epsffile{Scheduling_example.eps} \caption{Four-processor decoding
schedule for an IBPTC where $z_{ij}$ indicates that the APP
decoder $z$ is performing the $j$th decoding round of its $i$th
decoding phase; each arrowed dashed slant line from upper-right to
lower-left represents a decoding phase for a certain APP decoder.}
\label{fig:scheduling_example} \vspace{0.0mm}
\end{center}
\end{figure}
\newpage
\begin{figure*}[ht]
\begin{center}
\hspace{0.0mm} \vspace{0.0cm} \epsfxsize=160mm
\epsffile{decoder.eps} \caption{(a) An IBPTC decoding module for 1
iteration; (b) An IBPTC pipeline decoder. $y^i_k$ is the received
sample corresponding to the transmitted bits $x^i_k$; APP$^1_k$
and Ex$^1_k$ represent the a priori and the extrinsic information
associated with the $k$th information bit $u_k$; APP$^2_k$ and
Ex$^2_k$ represent the a priori and the extrinsic information
associated with the $k$th interleaved information bit $u'_k$.}
\label{fig:decoder} \vspace{0.0mm}
\end{center}
\end{figure*}


\begin{figure}[ht]
\begin{center}
\hspace{0.0mm} \vspace{0.0cm} \epsfxsize=80mm
\epsffile{partition1.eps} \caption{Partition of equivalence
classes into subsets and IBP interleaving; $L=68$, $\Lambda=27$,
$T_c=T_s=3$.} \label{fig:partition_example} \vspace{0.0mm}
\end{center}
\end{figure}

\begin{figure}[p]
\begin{center}
\hspace{0.0mm} \vspace{0.0cm} \epsfxsize=120mm
\epsffile{w4_error_event.eps} \caption{Pre- and post-interleaving
nonzero coordinate distributions of weight-4 input sequences that
result in low-weight IBPTC codewords.}
\vspace{0.0mm}\label{fig:w4_error_event}
\end{center}
\end{figure}

\begin{figure}[ht]
\begin{center}
\hspace{0.0mm} \vspace{0.0cm} \epsfxsize=140mm
\epsffile{IBP_procedure.eps} \caption{(a) Inter-block interleaving
using a non-swap structure $(S=1)$; (b) inter-block interleaving
using the swap structure. When one starts to interleave (or
de-interleave) Block III, Block I has been completely interleaved
(or de-interleaved), its content was dumped and the corresponding
space is emptied and becomes available for storing new content
again. The storage spaces enclosed by dotted ellipses are thus not
needed.} \label{fig:interleaver_procedure} \vspace{0.0mm}
\end{center}
\end{figure}

%\begin{figure*}[ht]
%\begin{center}
%\hspace{0.0mm} \vspace{0.0cm} \epsfxsize=120mm
%\epsffile{encoder-IBPTC-TB.eps} \caption{Block diagram for an
%IBPTC encoder.} \label{fig:encoder} \vspace{0.0mm}
%\end{center}
%\end{figure*}

\begin{figure*}[ht]
\begin{center}
\hspace{0.0mm} \vspace{0.0cm} \epsfxsize=120mm
\epsffile{BER_402_BW.EPS} \caption{BER performance of IBPTCs with
SRID $\approx$ 800, block size $L = 402$ and interleaver span $S =
1$. For comparison purpose, performance of the classic TC with
$L=400, 800$ are also given.} \label{fig:BER402} \vspace{0.0mm}
\end{center}
\end{figure*}


\begin{figure*}[ht]
\begin{center}
\hspace{0.0mm} \vspace{0.0cm} \epsfxsize=120mm
\epsffile{BER_265_BW.EPS} \caption{BER performance of IBPTCs with
SRID $\approx$ 800, block size $L = 265$ and interleaver span $S =
2$. For comparison purpose, performance of the classic TC with
$L=400, 800$ are also given.} \label{fig:BER265} \vspace{0.0mm}
\end{center}
\end{figure*}

\begin{figure*}[ht]
\begin{center}
\hspace{0.0mm} \vspace{0.0cm} \epsfxsize=120mm
\epsffile{BER_3G.EPS} \caption{BER performance of IBPTCs and the
classic TC with SRID =1320 and the 3GPP interleaver.}
\label{fig:BER3G} \vspace{0.0mm}
\end{center}
\end{figure*}

\begin{figure*}[ht]
\begin{center}
\hspace{0.0mm} \vspace{0.0cm} \epsfxsize=120mm
\epsffile{BER_SR2.EPS}
%\includegraphics[height=3in,width=4in]{BER_SR2.eps}
\caption{BER performance of IBPTCs and the classic TC with SRID =
1320 and the modified semi-random interleaver.} \label{fig:BERSR2}
%\vspace{0.0mm}
\end{center}
\end{figure*}

\begin{figure*}[ht]
\begin{center}
\hspace{0.0mm} \vspace{0.0cm} \epsfxsize=120mm \epsffile{BER.EPS}
%\includegraphics[height=3in,width=4in]{BER.eps}
\caption{Influence of the interleaver span on the BER performance
for various IBPTCs with SRID =1320.}
%\vspace{0.0mm}
\label{fig:Interleaver_span_BER}
\end{center}
\end{figure*}

\begin{figure}[ht]
\begin{center}
\hspace{0.0mm} \vspace{0.0cm} \epsfxsize=120mm
\epsffile{BER_com.EPS} \caption{BER comparison of IBPTCs and the
3GPP defined turbo code of various block sizes.}
\vspace{0.0mm}\label{fig:IBPTI_3GPP_BER}
\end{center}
\end{figure}

\clearpage

\begin{figure}[ht]
\begin{center}
\hspace{0.0mm} \vspace{0.0cm} \epsfxsize=120mm
\epsffile{corvariance_ext_in+ext_o.EPS} \caption{Covariance
between a priori information input and extrinsic information
output.} \label{fig:corvariance_ext_in&ext_o} \vspace{0.0mm}
\end{center}
\end{figure}



\begin{figure}[ht]
\begin{center}
\hspace{0.0mm} \vspace{0.0cm} \epsfxsize=120mm
\epsffile{SNRio.EPS} \caption{SNR evolution chart behavior of the
IBPTC and the classic TC at different $E_b/N_0$'s.}
\label{fig:SNRio} \vspace{0.0mm}
\end{center}
\end{figure}



\begin{figure}[ht]
\begin{center}
\hspace{0.0mm} \vspace{0.0cm} \epsfxsize=120mm
\epsffile{EXIT_CHART.EPS} \caption{Exit chart performance of the
IBPTC and the classic TC at different $E_b/N_0$'s.}
\label{fig:exit_chart} \vspace{0.0mm}
\end{center}
\end{figure}


==> conclusion.tex <==
\section{Conclusion}
We present a class of IBP interleavers that enables an iterative
decoder to collect information from a large span of neighboring
samples with a bounded SRID or average IBDD. We derive the
worst-case codeword weight upper bound for the weight-2 input
sequences and provide constraints on the selection of the
associated intra-block interleaver. The codeword weight
upper-bounds for the weight-2 and weight-4 input sequences, when
we have the freedom to select both the inter- and intra-block
interleavers, are also given. It is shown that these bounds are
better than those of the classic TCs with the same SRID. Our
analysis also indicates that an IBP rule that possesses some
regularities like periodicity and symmetry is likely to be a good
IBP though global optimality has not been established.

Using some of the properties and bounds we derived as design
guidelines, we propose a simple IBP algorithm, suggest a modified
semi-random intra-block interleaver and address some
implementation and hardware architecture issues. Simulation
results based on the 3GPP standard turbo component code show that
the IBPTCs provide 0.3 $\sim$ 1.2 dB performance gain. The
performance curves have sharper slopes in the waterfall region
with respect to those of the classic TCs with the same SRID or
average IBDD. The class of IBPTCs achieve the same performance as
that of the classic TC with a much a reduced SRID.

The class of proposed IBPTCs provides flexibility and tradeoffs
that are not found in the classic TCs. In particular, it possesses
some desired features that suit high data rate applications
naturally. Since it can use any existing block-wise interleaver as
its intra-block interleaver, the encoder/decoder structure is
backward compatible in the sense that the special case $S=1$
degenerates to the classic TC structure.


%\section{Acknowledgement}
%The first author would like to thank Prof. J. Haganauer and his
%colleagues in LNT-TUM for many hours of stimulating discussions
%during his visit there.


==> simulation.tex <==
\section{Simulation Results}
\subsection{Error probability performance}
Computer simulation results reported in this section use the RSC
code of the 3GPP standard, $G(D)=\frac{1+D+D^3}{1+D^2+D^3}$
\cite{3GPP}, the interleaver of the same standard or the modified
semi-random interleaver of (\ref{eqn:semi_criterion}) for the
intra-block permutation while the IBP follows the algorithm of
Table \ref{Algorithm1}. Each simulation run consists of 1000
blocks. We use the Log-MAP or MAX-Log-MAP algorithms for decoding
classic TCs and TP-IBPTCs, the sliding-window Log-MAP or the
sliding-window MAX-Log-MAP algorithms for decoding TB-IBPTCs and
C-IBPTCs. In most cases, we compare the performance of classic TCs
and IBPTCs under the assumption that either both codes have the
same encoding delay, SRID or they have the same average IBDD. As
discussed in Section II, the latter implies that both codes use a
single APP decoder and identical block size $L$, and the former
case implies that the classic TC uses a block size of $(1+S)L$
while the IBPTC has a block size of $L$.

Figs. \ref{fig:BER402} and \ref{fig:BER265} show the BER
performance of rate 1/3 turbo coded systems with 10 iterations and
Log-MAP algorithm. The interleaver parameter values for the IBPTC
are $L=402,\ S=1$ or $L=265,\ S=2$. Compared with the performance
of the classic TC with $L=400$, the IBPTCs yield 0.7--0.9 dB
performance gain at BER=$10^{-4}$ and 1.0--1.2 dB gain at
BER=$10^{-6}$. When both codes have the same SRID, the IBPTC
provides 0.4--0.6 dB performance gain at BER between $10^{-4}$ and
$10^{-6}$.

Figs \ref{fig:BER3G} and \ref{fig:BERSR2} show the BER performance
of rate 1/2 turbo coded systems. The MAX-Log-MAP algorithm is used
in this example. We compare the performance of the classic TC with
$L=1320$ and the IBPTCs with $L=660,\ S=1$ and $L=440,\ S=2$.
Using $L=660,\ S=1$ and the 3GPP interleaver as the intra-block
interleaver, the IBPTCs have 0.4--0.45 dB and 0.3 dB gain at
BER=$10^{-5}$ and $10^{-6}$, respectively. For other cases, the
IBPTCs give 0.4--0.45 dB gain at BER=$10^{-5}$ and 0.4-0.6 dB gain
(except for the case TP-IBPTC with $L=440, S=2$) at BER=$10^{-6}$.
It is clear that the IBPTCs outperform the conventional TCs with
nearly the same SRID. Furthermore, the proposed modified s-random
interleaver outperforms the 3GPP defined interleaver, especially
when the interleaver span is small ($S=1$).

These figures reveal that the proposed IBPTCs yield superior
performance, sharper slope of the BER curve at the waterfall
region and lower error floor when compared with the corresponding
performance curves of the classic TCs for a variety of different
code rates and decoding algorithms. The improvement is more
impressive for smaller SRIDs, and with the same SRID, a larger
interleaver span ($S$) leads to better performance.

Fig. \ref{fig:Interleaver_span_BER} shows the BER performance of
rate 1/3 IBPTCs that use the 3GPP defined interleaver as the
intra-block interleaver. Either the Log-MAP algorithm or the
Log-MAP algorithm is used and 15 decoding iterations is assumed.
All these IBP parameter values, $(L,S)=(660,1), (440,2)$ or
$(330,3)$, give the same SRID of $1320$ samples. The performance
is consistent with our prediction: the larger the interleaver span
is, the better the system performance becomes. The performance
deteriorates when the period of encoder, $T_c$, and the period of
the IBPI, $T_s$, are the same. For this case the lower-bound of
(21) becomes $2(1+\alpha+\beta)$ which is much smaller than the
corresponding upper-bound given in {\it Theorem 2}. By contrast,
the two bounds are much closer if $T_c \neq T_s$ and both bounds
give identical value if $T_c$ and $T_s$ are relative prime.

Finally, we want to show that the IBPTC requires an interleaver
latency much smaller than that of classic TCs with similar BER
performance. Fig. \ref{fig:IBPTI_3GPP_BER} shows the BER
performance of rate 1/3 turbo coded systems that employ 10
decoding iterations and the Log-MAP algorithm. All the
interleavers are taken from the 3GPP defined interleaver. The
average interleaver and deinterleaver latency of the IBPTCs is
about 800. It is observed that the performance of the IBPTCs is
bounded by those of turbo codes with block size $L=2800$ and
$L=3600$. In other words, an IBPTCs achieves BER performance
similar to that of a classic TC which requires an interleaving
latency 3.5 to 4.5 times longer.

All these figures show that the TB-IBPTC has the best performance,
followed by the C-IBPTC and then the TP-IBPTC.
\subsection{Covariance and convergence behavior}
Fig. \ref{fig:corvariance_ext_in&ext_o} shows the covariance
behavior for both IBPTC and classic TC with the same SRID, where
the IBPI has $S=1$ and SRID $=800$ and the interleaving depth for
the classic TC is $L=800$. It indicates that the covariance is
small for the IBPTC even at SNR = 0.5 dB while much higher
covariance is observed for the classic TC at much higher SNR. The
IBP collects extrinsic information from farther and farther away
as the number of iterations increases and we have expected that it
results in smaller covariance.

Two similar techniques have been proposed to study the convergence
behavior of iterative decoding schemes, namely, the extrinsic
information transfer chart (EXIT chart) of \cite{Brink99,Brink01}
and the extrinsic information SNR evolution chart of
\cite{Divsalar01}. The latter is a simplified version of
Richardson's density evolution approach \cite{Richardson01}. As
the extrinsic information in the iterative decoding can be
approximated by a Gaussian random variable, the evolution of the
corresponding probability density as a function of iteration can
be characterized by the SNR evolution where SNR is defined as the
squared mean to variance ratio of the density.

Fig. \ref{fig:exit_chart} compares the EXIT behavior of our
proposal and the classic TC with the same SRID. The IBPTC yields
mutual information almost equal to one at SNR $= 0.5$ and 1.0 dB,
but the classic TC needs SNR $= 2.0$ dB to achieve the same
performance. The SNR evolution chart shown in Fig. \ref{fig:SNRio}
exhibits similar behavior of the two codes, all indicating the
proposed IBPTC gives superior performance. Both figures also
reveal that our code has a much faster convergence speed. The much
larger step of the IBPTC curves means the associated APP decoder
generates more information or extrinsic information with larger
signal to noise ratio for the next stage decoder. Such a trend has
been expected when we examine the factor graph structure of the
IBPTC in Fig. \ref{fig:factor_graph}.

